Towards the Right Kind of Fairness in AI

Fairness is a concept of justice. Various definitions exist, some of them conflicting with each other. In the absence of an uniformly accepted notion of fairness, choosing the right kind for a specific situation has always been a central issue in human history. When it comes to implementing sustainable fairness in artificial intelligence systems, this old question plays a key role once again: How to identify the most appropriate fairness metric for a particular application? The answer is often a matter of context, and the best choice depends on ethical standards and legal requirements. Since ethics guidelines on this topic are kept rather general for now, we aim to provide more hands-on guidance with this document. Therefore, we first structure the complex landscape of existing fairness metrics and explain the different options by example. Furthermore, we propose the "Fairness Compass", a tool which formalises the selection process and makes identifying the most appropriate fairness definition for a given system a simple, straightforward procedure. Because this process also allows to document the reasoning behind the respective decisions, we argue that this approach can help to build trust from the user through explaining and justifying the implemented fairness.

==> urls/study-url.tex <==
\href{https://axa-rev-research.github.io/drawio/src/main/webapp/?chrome=0&grid=0&toolbar=0&p=props&title=Sample%20Study#R7T1Zl%2BI2ur%2BGM8lDcWwDBh6ra%2BnkTnpJd890el76CCNAKWMR2S6q8uuvdsuyDIYyW6cy99wuvMiSvn1Vp3ezfHpLwGrxDk9h3Am86VOnd9sJgn5vNKD%2FsCvP4kowVFfmBE3FNb%2B48Bn9DeVFT17N0RSmpQczjOMMreRF%2BVyEkwRGWelBQAhel9%2Bd4bj81RWYw8qFzxGIq1e%2Fomm2kFdDzytu%2FALRfCE%2FTSck7yyBelpeSBdgitfGpd5dp3dDMM7EX8unGxiz7VMbI967r7mrZ0ZgkjV54cN%2FJj3%2F3%2B%2BmfTQbB4%2BD6%2Bv%2F%2FPHfq0CCI82e1ZLhlO6A%2FIlJtsBznID4rrj6huA8mUI2rEd%2FFc%2F8hvGKXvTpxT9hlj1LcII8w%2FTSIlvG8u4MJ5m86bPf1aXI1aU4J5Gc1104%2FfCWLP6eXf8fePq%2BvvsW%2FefuKpQ4AcgcZhvWORbPsbUZH5Ab9RbiJczIM32AwBhk6LEMfSCRaK6f069%2BxIhOOfAkxl8F4Xjc9byx%2Fm8khpD4f%2BWPQq88qFiiHKcAH%2F3DmFhxiQN1FwDLHXoEcS5X9Y0SlAvov4EJJd8SoECM5gn9O6KAgYReeIQkQ5Q8ruWNJZpOBU7AFP0NJnw8hhUrtiC%2BxMGbzuC2EdA3Yij7MnwqwUUSvfxqiaxKQFXA8bp9L%2FRLAJG%2FXgr28qD98vt4NkvhQYDr%2B05AHph6KbzI8x%2Fs%2Fe5A%2Ffwmh%2BM%2Fbp9Kv57VryeU%2FWH8%2Fa0Ygv4qXmI%2F1DvtcYqgIacYHoRTXBMCno0HJHlsYCTD%2FtBmHb5nIZEYtQ4nw3HPGiHsH4z5%2FL66Hq4971c4%2Bbp4Px1%2FvP4wfHOllnCxzEcRWCvMZzjyBmWA9FvhPr3yqC1wHzz5kylTgRcLqNzy14Ot7KhvTFLix2WxJv9cWJPzuf6xlJggtNWWsG8NU8M5HIP1tg8mVr4HG6I%2FJa7uIjWVRlFwpff4kphSvy2m5HW9ca%2FXjgo0HB9N6%2FEq8OsEYUy37M2kBMPwr5wZV3yfr1K%2B0df0Ad9fPfHdVvfpX3P2791fOeA8C8Z0ExFOBDRQ9qzGp%2FOdqKcrGFNwLwbM9QJl8PMKcMpfU%2FPYMoFQHN%2FgGBP%2Bbm82YP%2Bj19OM4Ado3An5f3IVxnXx3y58qIIv9cIqGI88i2j9QCLK2rCDlT6xMEzgnlePOyVU2CxvFEkSCFKcoGRehvQiUHD4pB8ogFTcVRdX6sJXyOeW5kv2R7YA7LsJZluGYxQhpp94lNGn7DoFYrRg%2Fgu4BMmU3ZAoMocU1IRPb0UJnW41kAiDEj4sG3xOyYn9SsFyFbMLKeUaFJ9w15jqqoxPmzF%2FeHIBu4cOv69QthFbO1DYzT%2Fz5UqtNcEJW1z6ALNoIe%2FvL42Vm2mbNA4aSuNCAez5ftgOs6Ws2xaqQ3uY5hK6Olg4bCahdzdreqO%2B9a2x51usYZNZY81rHymzl9IQnMbU3kMvbYvc9qegXpWCjmhqu2zpYbDZKTc8slMuqGgwHwleUQRBDD0uSBet1S32MZBt%2B%2FggzrnRuKtU3sOrqkpnuiwr%2BDQOuqZcQ6n%2Fh2cbo6Etq%2FoNGcXucnHs2wq3%2BpZTLraGoMqWLDiRsoKSfDmB5JK8dYra2jCM%2FcELnXMKjqN%2BNwzHxn%2FH4j39auTnI4ERSrmd8sqVmnGlcZUrOZ9rqssYsahhby8BtztvGflWIGA83imSQOdkD9CQD7oMgMAaa2Q7DGpsjWKsE7i2%2B2djeV%2BWKdCUfEY7k89w0I52GPhbEbI5cnv9kyL3NsvWGaQbVOXEJ0jl9iWZITrQ2IYZ4vdGYQmKLdkhvcA1aquKgDsKe1FGyF68x4kUvWFD5jNoyHwaI0CNm7shuKoq%2Bec8iiBk4DhLktyIda2QZNhT4aWWQ%2BeBdgZYAx%2BBLC8n9e5l5BWeF3lVxd09QPFl0VabOXGjwdiirZbkXX%2FQDcs5TIcQeRtx0wCygCT9eJJgFayzAF4mrm0B3EOEXf2Ka3owlFqDGXYNHGFXO6%2B0PYLxKht1Aj61rzqxP39T6z4%2Bf6uzLgYD2x%2FZ643Kw%2BydSdMQF4IfgHmq9JFWFJPQLzPPoB3e6Y9t3qnizYdXTAbjcyD4IxBu60UBL%2BKzYTWt6RL1foU9LaXMhi9080jq6R3P7V4Fo1I9IkyISiw7O9Wj75XdE1d%2Bf%2BDI%2BGpJ9djTDTswMeZiEqCOqstscq9u5Yh%2BcCxdxq%2FY3Q0Lo1zhibGlFw2CZl7XPdKXAitMq%2Bq59ozS7pWLNFDkXbCYmxikqSans5QWGwi6JWnhBZbjVulML8RWlQynOWNArebwWAJlEJxCHbvMcFNjPtc7Fp8LvGF33Pf9YdgfeoPRqLVYkz%2B2MylVfdgBjEE3YioPr6GwUhUHXhL7UfZsK8Wlvu2kbiuBzeY%2Fx2I94UVFjk5bxKVUp635a%2BHRdCytmGsdqyG3aQ1%2FRhUOcQ%2FilJVCrHCK%2BOIuh1mELaaXBeORbW61wivKnGJI0X%2F4cmaxp7EWXmw5aMVg28PoOwYnOVombKVqo9daxvxeFlDoCuIJxpLAuVgro0FZFUhKmLdrWWAnoP%2FnXTLjaq1glBUxlflWSyrOcNS1bLfR0Tx24UkC8ZqnaD7yzbhzro6k5rzJPxpvsvP3Atv7s0tyqqUx9Q5nU40G8x55enh%2BO34XR%2FD%2B71sIoasyqMrYjs94mjKaNvMS%2FNHAmT3w0oT8o1lPKrHyMnSe06bZ%2B02rf1QI%2FOT9eTxbJRr2d0uq9%2FpWrsewId9qDT9VpM4oENHKjRcJj%2FLFKDk6jbkF66w%2F6LdaiVgUmlLD7wDsJ3v%2FB5l%2Fid%2BEn76nk7X%2FNR0%2BDVR0%2B9Vt3Cb3aT1VeD%2FuQ2WjzTyOxX2aTCY8nNbkRHVHR5j3hRl4xpxsE%2BG2097HO4xLuqxyB6NW%2FEzNxNZw%2BKpWNWZsh%2FEQ7dHN0A6N7MqvwtBSt8LeuKvi%2FrsbepX5DEbHDZ4Nq8qX04N14a6nYWuFWax9jqop2Zd7HYE5jV61rl2Z0%2FY%2BMYfRulxcxsrmvQq9l3CZfpVpHSoxaWAL%2Bo0Mti10H1UVr0tmVipc2YqfvAyOoBW9KyibpcNRV7XMaZW1OV2TJ2mA9QLuUmUum9rOHD8J3O3%2FrdDTiRomVzd%2BE1K0U4imG1a%2FuPKsBR%2BvK%2Bj9kXWIpI%2Ffi%2BGnMI0IWvGEbn6%2F2pxSvtGoM%2BUt5r0nRe9ImDwigpMlTEQfSkjY1WecMwyi4OXdKDPMZ7GK8bN%2BEaxW9JO6G%2BWS8mF%2BOcnQ1RSxCS9Rom7rlpdsSd6XhXh2yWVPmsEl%2FWdG8JLvwroT3HDYzPNYvY%2BJnA7hbcvo7zlIUApUHzNxfkeMEpjW9Ly09uCejwifZMfMG70s9SSgfy8InPENV5HaRZax80CuGXiD%2BxnprtEDWsEpAl06I3qJ%2Fab%2F%2FIbRd4Vb3zvB4Ibi2%2BDa%2Bx6D76yPp74y1g09i6fGf%2BUoRhPjIfidIsD3GVwu6T8w478WmP8C%2BfcUooRfooRA%2F47T7xRig2AIpnT%2FUZoRMT5%2F73uak0f6TAwSytOMALTJvtTV7xP62IMjTH0XdKg8Ht%2FcUN5Kp3g9vvoforMhS5Ak6uatAqWGBShgQWFLF0kMLJxgQKbsJ54xHJIpHDh64ECKFiCZs8diuh5WpCLwIaVbB6%2FwOuGXIrxcUZzgg%2FLeqPdErFJgL9sd0WtVfIJTHAT8CtNgBurOmtJqUoNEUgtRnLVeHtQmoxAKuElOcWhb7cUUqRIOehemKo%2FA1DZAuhJH0czQE5N97dRnhLaTzR%2BrPHCzPkMdP2PWZ%2BiLO4grKy2jPgWo7f68H3KOQ6pl7hRkjOTTBTvKh66A%2FR2zpcVsdxb0L9GGl6KcwpQZAfk0jwXnjGKAluzNNJ8sUSbQdMLeXULRqRck6opCMe8zLigAcJYox0dspCmazSCDJXv0F7yGj2wKjFWt2TMLwE133lKYFJxQ7JNCe7sBsZiMfBWIPsIRe4XPl7F7mETP%2Bm0OimKd8XOxEr2IL0xmzHg%2Brp4byDKCJnkmvixXQ2UCpCTKhze6F8ud5x%2FMkzUVIGLvEGC83NvewtipMAw2kuFZa5RBQ43yMPXAbbTaDUfWEVENSoytd9oucHEiSTW7i3UDZ1hMcVdwgzzmyHgm2RD1qN6Sbjz2R0fojRrqouO2NWfVVFKyUzMzT7AOxmDTXTRra0TxfiMJ86WOsQu%2Bt9KdeLVSEmXiW8qnkSpVR99RPlt%2Bh8sDrcdniAh%2FyErqzVzC5LyvPKhMJBLiiL8qVwgiglMpwjrsoDycU22Xk4PQv7PyeyX59CtbgDAbEkwRHnK6Is9cHlubJ7g%2FfZho9n%2Bj35aySZocEVXr2QvF6ExA6FXPACJU5%2BfyBc6oviu3k79NpVIsEMQpgvia6FylDGOjYbLkW2pAKRIzp4ZRoqeghSrgD%2BSpFLxi29MFWvEtytYQGk362XZyCczbnYqHRLN%2FlwYg7sglSy4UowdYbNzGtWfgwZC9lBaFOI%2BoVDMWTCec8QWvDT7HLDuKmgRJjC22fpvGseJjpRp8lCoRfDS0D2MnUvE823ITlbiGIZgv%2FYLQucrKhKEyRDg2DtAgOBK7wQGL5cvyUQ4crleI2aYC3MWIagIWsrK9%2Bga5Tz9RQ5Y1rEgas4qKFI6DVAyFJAnBR4kMOJ8v7JWk%2BXwOhXXCPrJGqdSmOPgk8qmZlvSotCNtmymdvrbVMUFzZn1zrBaGNcWEjF6O%2BCTLBrqm381EpaUhVRnjfKrBvBS4xrFb7GkquE6KI8Q%2Fh5I%2F81QyBUPzW3Hz60ZRlGAV0MlvqZ0Rc5zhX1zlabGFTE8jFF0fUQznfAs4gtX5AToBy7V0sOtfE0nRS2rQi21S52iYDgJrXmLBXBnWVCs1fsx3guFVAYUporJKIggx0IZrzgvETRHWJkmboxMijdSIWbMcs6MoJ5qLajX8WkJOfGSeYLbhHdtPo2EIoocEr2OuPLoYJMcJtSOc0PiDzKuQpnKs0u4sTAOljpzUrM1hmBOG74cSP%2BbLMFskfBmaaUQlVqVYg8b8PFEIhFdMvOYMfQUdGyhOBUsMBL0ILUKEQfF2IkAaCWWXhc3ofiM4BJXnm5DbEKqCGyChs0leDKJFg5Nc6m2Jl3sjjuN66Pdso0CfYnoE10Oz7imqLOHykvj3N0j7VYN0Yze0M2l0ozo%2FmD3nqRBmmnT8fAp7bs9ONwrlWsltGKpOXi3kmLZxvsX2mj%2BnzTs%2BtXvn%2BCUxDio8TrepWr%2BPakGkUcKzz31tK%2B3AH47tb231MTne8bf6pXqq81zdO0fxSznyTM87PNtmL65RJTmmHR%2FUYFjpwXug8G0D%2FuVvDhOdtX%2B6KSM6Vj%2Fe%2FUhMCdVTH87akMJaPSF63PNaOiAwbKHMxEVCbzl%2BMywjecY9mI8AxWKJzX239ihur22tR%2BAdNbxQwh1lEBARWvRAPMcEZYtlYcNnBKCkCPjJrILCzca9G6uSAWn6w%2FiydfBbXONDig9KF5H4lDY6pUPiWcCfWpuZ6SBL8xXLx1DOkGIP2KRu4QomUzE4rsThOPjE6MiyTec5ICw8x8ZlT8zKSRRlP5VeFSWBPBZxRO4CMQ3uJQRpTiDLPtGeOwHXifAVTVG6ypUxPANRllaDoeKrxvdW4qTUjuX0WuRLvpapPJwoLe3iUmkkLIQZizaKSQa4u0K9qWKS12l1mSkkIqgq5sA9GEX6AaQQWgIDQks8hfG%2FhN8jygmICscniFOs3mMpLumMz6xTckowcuKOEb3pHFo40VEGOv0p91pUIC2btxU%2BLUlcKOZHEMtghOAOSO793CZI5vXTkXLK9dCMbjPfdOW%2FiWADH9z%2B7jgejuArpaieIjFNlesRxXlKUYy7k5mrB%2FE9RGphWb4UTnT%2B%2FgQmjG1L%2FFty7i6Wwuk5Aw%2BS9DkK4FXK4cF3Q7qwi%2Ft0GzEBFOkUJzB8rL8IjCj2vbKpfDqa1RU%2BOJFiBbgLjtI%2Fnmt%2FVNm9p84RVt5SXpIk1g4SOkAscZ4jdEHd0oNbZTocE%2BYYszky15XAj4IXqxQHkEijWuBWLAaputaZ20h6474KvKW0SsGbiRfYsWFT9IjS5fZdSjCH%2F5KhByWs2J5YigT5gTKCJHDNli2c39xNSGcnnlRBEBk7WcXAdljP8iwnRXRGsAwxEenen4iYUT5fZPu67DZ3szkzl50%2FqpwP3Ds3l93gtIVc%2BodRLXGUuodBVU%2Ff2En4TNx2g2ozrxMZv%2Ft2pm7zkKiiM3W7CRm93hlZw71TG8PH9%2BY5iPOI3rw9CsHt3scX40xTTakuxNBv8zircTAsN7sK2mEeZbC20fPexThUO3tmde1i9Zfe29Xml2opz3GpKJ7widqTqdb%2FSsZTXLIGhbU%2BkXm12DI7tZ6%2BFuUWKKEaMik8CEo9r5inF26SlvZD2iaF8SKj4WXbLiK5jKqLXBNq98yBmVe8whnLfRMGouC6KnVCbM3eFqijRoQbkCmeZWsB4CIbgHuI1A%2FDhbFa4AxzkCOOQmvMCx0kZDUk2RNzmEBiAqRqj0l7dD4XV3X2OrcNU%2BFxEnMC6QOHWyzy2YWrhudyUMYiUGgK5wTq3WJZ4NIrM6OXp3jpdvIY5lAKi%2FQrPoagYu3JoU%2BhwqOzUmbwHbcCpb2IZgUoAXMLCRMTGflhBV3gJFZ4ly5FlYhKq%2BPfX0FslfNUt1AQUpHCZBHSXibb5mTz8zLZ%2FHHfluT9Ye9oJtuxCzx0qiBnnMJx0OGJwbKsCT5RQ1%2FhyCMg3OGVloqjFLdWqUc8u2dWlMJNYUbXVKpa%2BCrTe0TGYJoLSDLewRNHU6qjKqQ1qUiILJU9qT%2FAckwVB6L6J57mEf%2FaNCclT8vmtMha73IDtHcnJowuVW9vz8gOGxrZx0qN2S%2Bpqdok5DQ68r4ZMm0W1IfD4IUpMq0XNbhZ1C5FDHVMrgEf%2FWbm6Vf0UGMwzSdVqMrISo7hHGl1UxCV5kl21ums4JMPiCva%2FDEkMjuFfuDMrrfCVayWr0jELVUZZzJp25i9EfIyuXOllNn4QGmFUo6ovE0%2Bb6pHwxUVDDvnIv8Gs3%2BJSoyVrKtOQQwEg2C1sEbsUYsKpc%2BzDwul7U%2FM6jhkhCBxhM7qdCS2cx0dpRQKvFK0qAL7wDVKuOaybYFFNrKIRtChgcwoBgV0eFK7jmbowKKSacCARKco2mEAE9vBvkkn%2BF1%2BS%2B9l8YQhnUtWj1O676vmhRek5gWh1%2B969oEePdWx4Hyc8ydp93GZR380PQi7%2FW5sL3PoVz1wF3CM2EZsbUXRGPR7h3Dt%2B94xjsN2b09wicR8mpaJDmJ29zo%2FWj7vWLXF0b0KWzt8oyH6VBP2z%2Figr40U0I4lMrAOwWjHfd%2BzQva9wcHKsT%2Fk2Yo7kLPnFdzFYCm%2F2MhOYQVwqUAXmUcjNj1DSY7zVOOVKGieZTJfQ9kRntbafV2OJ7w%2BXJE1s8p0%2FfakyJkyi0lXVndzrvkW%2Fnms1gYKCUitG2qhgKmpl%2BvEObEaNos8AcsJmsv1qIiC%2FrzQ1A1HD%2F%2F8nj2RZKUemyMGMtWI4EdHJhawd17t7ooHHWRgA0ovlpyaBIY5WzVGDMGj0RzI6L8kfbWGDzpmUsJ01knLkWBu6M2KzlF0MlmRiuXIIHTuOpU21KhiTIS7nqU7rS4DEulsLZzEInV0CcgDlPlNrnrSqKwKSQPbcP6Zm4hNstjXjBlekhkzCi2hNFba7Ymc1a8s7ZWlvbK0M2NpmwMRZ8bSKjmTp2ZpatPTFYdzsxPsKn0B7xj6Ky9ptfGOzg5YYt7PgDIezVK4E1NnEjCear9t4IWYpYkaTfpjkoKxcAT%2FBCMeQG7Chj%2FTmT%2BYgTbCQcLyGWQnRYPprowvCeZL5KcKFs4KDK5Y%2FwUZoaMmwVKR2rJSdMKI25y%2Fyi4o2MmMgFIcXnFrSd88w5oTG2PJbMaOHBTRYki8IV%2FvGvtk9sSxP1fpW7T5S7KGRYT%2Fpyx5Y4b47IBwefNuB94v%2FGHdUQ4K7ILGcCLJA4tqBI5dqZrnUnDdehwrMdw5Esnbgpczv7SRoC5ZGmuu%2BVcOEyNuAcorVpnsfF9Uh72O2WafLWbFG1KILVquRIM9ozSDVbw8oqnuCSKbOy1XC9FJRqWRUJYuI8qVdZnSCpcwsrKqsmDQ4eoJTOAM6WYW%2BnG2ndK3n3Ear0y6iEswuYqmHKysGKGjE5lUlr3R6IbJnLmUIHUrqYOoIK5WCk14n8OOCufbPU50b1yK2blqLaq7PtrBGJQ8snjMXMZjROsss3NJKXYk%2B7aIRCK0RIVGluSsW5TCuDXByZzTjcwoEJ1PKcKWktJUO0bKS57oaCnsWGyJFyz8pcidNbfk7OaRS2uZKiSEaD4RkbWiFKWzXXmSXAJHuUg8mwMiy80M6JZ2Q%2BR%2FSVZzU6CYap4kPiWrbJJNs%2Bf7xCZY9GlhdJmtmWPxuWOGw9gP1XPGSCbaOwtoc0%2BCM1NCeuOya8ko3j%2BRFnJHiDA4qB6YOvSHitpgP1HVIppGx11fbtLbr9SpqDxIqQ1buf9awS5kpyH7IINSeumseloLSxJkBFlTyFmIMWkYcm3CnF%2BnpJM3EJbOaO4%2B7bUa2BGa0TJWI0LYWDbRQkZMfFrit6VYv9mLS3Xm4nyBQMomRGUf5SczpAP%2FRcmiVg0cYFHtmn5iXzP1QaAnozIQ6SKwhrOsEIvRnBWh%2FWzyHSt7wYCKyB1Q6QTcnMKC%2F1UVMa2SFJ9XaoJjwWbnMYZGHyzQMnLnm3fTMSzmmaiG21R9KHUxmxJKXVQNzh3zJIOSuKFMWq8lfRCqBxtlA0vOMI4ztFK0vZVL%2B94lsemhbyVr6qYml20rts%2Fr27YYX4XCq1B4FQoXKhQ2S4DgkiRATwXhlQToD48nASpx%2B43H2hpx%2B68q0iBdwcjJ5W0W00yjbwNWrYDGs%2FtVHlQ471A5YZKAM03hbNvn6XttJu47t0D64Lcn03VaTr%2FZX%2Ff6%2FOX605fGCsxnurSsmeLyRjmMRJ%2FvSKp2RJaDcWZsCH7Z5h0W4pa3yOVKjdFdvJrHe1%2BMccOO60lrk3lVAxPxqZTiUlwoR4YAg9lCNof5K2cONyH2zP7yyrnLwqbwKdM6QAzBtPhCVpzEIpXPchf0unbAYm%2FkpwzB1yw8eUMfZ2V6hp5Gl6a6IZlnpCAwJ6CI%2Fs1yIoUyT3AWyemFD5Aqe7M87ugwXhNRWU8k9ZKyxAVOwYErhxUFnuq%2BsI0F260qD5Xg7Gg0VxFjIrf%2BJXu0e3pZ4NuZFYFDsQh6jq0Ld9%2B6Zsd8hq69kkpBp6mxyenMsjc%2FytjMo1Y2eYqDpomJTaIv%2B5ypybQwTHmCtgqkidBvQIQojm9wTHkIe7c3G7D%2FMWs%2BI%2FgBGndC%2Fp%2Bcq3Fd%2FNcIVTdTQ2MiDxwq1diBlPaJt%2FsgZfb%2BDzL%2FEr8JP31PJ2v%2Fazp8GqhEXQMnP%2F7UuRl03oR8U%2Bn8hswmEhnH3Dy6Zn8yi44%2F7jV53P%2B5AlgurbZCtJLzenjAPJc3fBu3aAMw7ikPKpA5D84aBpZdoA99PxlnHbr2qnXOSvfzla%2Behq%2FWHQJWRdNj0KuTkVa9BB9%2F%2BlZiiiafdDLS7Y%2BfnpE2h8S5MFIlYs%2BOkY7URIoGUoGjVcXgmJx0VK%2Bj0g%2FwBN0FIKl1mG6ezZgxZSZ1vph91YZgIsFX2CBkPvlpIMmj%2BPdnMQX%2BwRlYovhZPE2t7kfIMkON%2B44JyRviu%2BxOgskSxMa9tYQEu9n3hOufWtzstLErOu2I%2B6rsNxmdXiF2Aql801Pf43cyApKUnxcm30yguMta6pRH1S9OQPQgujhdWZsS9EdiN4L%2BWP4x8OS%2BsKbDMZB7gkRgQqwtxiCzPl8RiD%2FVRp5ewXZIsFXIREiHV2BcHg3Rf8GSSZtkkrJ%2FhLivmlWvsH0ltH84MA5FaEyP3pBAcTL1WuuqL1GvnRrjHur1pgSZl1m6t3CJ53QTF7xkYpNd3TAatGXArVktcwx0eu3UOZbjZIsZeMQ5kekKOM8i2f2sFPtnXSDnSRFLgkCcpihTj9VHxdkUSbkMrWMmM3eMM1tZHbdcCHtxQeCsBIdFlq1SDoN7%2Bn%2BAPKHHLiZz9veEjnrv%2B16%2F2xuzyLahs%2Btg4fdJDJIHB9hYpxoKVpMbAr2zg9vtYZj65mENwjCX4KnYgYAPQLF7hXC0SXtu9nEYjqs9flwm8sGcje79ajXktRkk%2B%2B%2FiyXyx1WZ77ciMG3XgiyjJYJWhaSaj49s9s7UKGtdnpPi%2B5prRLNusch3ebbtRIbkwfrhzREx5GE0EdkW42%2FAXul1g1YZOCjZT9FiPRE51eT%2Btd1ecYc9z3qDgVjyoIGgK%2BhmIyvMvjI12fHjOmCCFwC1sHkK0Hi9p7GK9hyI%2FDuXzMAcuL2wZuKjnDLQJf2wn0zjDli5OczBROThU2PKNrtwWCVVGIr00LF5jmEeXhP0aXK6XhA7TfnQgWnaGNKtHFd1Ry%2FNzpy4phJuAkqdvfNLnT56WtTYHxwbWeijFxD3lc80I8YcNWKszrelwrLVeiWuXtdqtg15Z6wlYa%2FOkBHl3XEXP4TE5q%2B%2FyubzaGLvgcVXA%2BI1FkW%2BLon%2BeZdFGHk9bmaqHCzTc8WTov0Urrun0krlzk6Le%2BtVujIDw0EZdDYhqAWMGIjKSu8t3xXWrbredkEXoe13Kx%2BpiFsXVuujFL4BMs%2FajF%2BGWivtzlaR71aNYmb%2BumgpfHcp34FiGU65WNeTa9PTn3bLZn8uuKK9zF3RGow5TdL1n4%2FeIv%2FWGGTt%2BZ3hEK2ev9gtWdCVwNMkJLovJr1aYZLwLGfwncfuaZW9n%2B7prH6vwfOKDURRKjf536s2igtH88oeynCmVOaquBvJgO1kCKEvlVWcBsw9rTURdFO8TKn0QsZog6Ir%2BH1e%2BmFT8Y8uXvvJ4bZQvLbnA9pIvYXP5Upfkv%2F3xYyb57wMl61wPt9RoKehwOKlxQ3drQmQfj9Nzc8d0miQuif0RujY2Dhut0%2Bb5TaXGV%2FR3Q3FfmZVPHN8LZi07lxjpSkUbxc%2B57MFtLKfo%2FaI7LnZko9R0hZOp7h2kJ6Y7daOiIalsrEr%2F%2Bkn2iJZXGHVVjtsVC4pUDx%2FdNFI2mlkg%2BFicvMoJR%2FVwFD1w2MlomJLFsx5L3cFLlKbGmb67S59VPlnCaTeJJqibxMtughbdOX6kd4Le2BsORz5%2Fbj8xdEPwOsXJAQTRlg6QP44g6nl2iaNTEIUnFESv%2FsPOi3MUyuV2n%2BmvtFFhnvVkxRxMO5Y5OJDm4I%2FuadyH0kY2pbmUCZfKt0eHC5cy8UX0hpO90uSREUKI7NBjdcMojYS57FstO62gKeRiMMFmH3K7d7RuaA0mmB8xYH9YtbCjoiwjaJKLqzcdV4sbfmh56dDnVNlaGzbo2pDZopezpAvRFTmuHM3MkNi%2BpFUCTtAiqEYws2dVsp9qafGSPtjqzFGqJuRL1WqPag8kR9lStDMst3m2ToqQx05wHUL07FZt9qTrc2204WOdcoyTSmVXP9Fl%2BhHJ9n%2FijfpR5Lvi%2BAxKgo8IrjtFh%2FGUJUByiM0h5eqkjCETINoFYt1OugARm8f9pn2WbfAy42sT4ddlR2mIg1o51iC2Gm64CzWwvBgsOx7WtQsyNQ5nc6reZoXjvDrZjdQx8zpVeeBq7nGsVnZOrSFwmK%2FSuWkXnde5R7c%2F%2FsO4R8eVRheDw7lHG54heKiMsXJ2tWinCqIoJyBiedWlMiq7w9A%2FOiFhH04xrtY1NO6h0gZqjQbzHnl6eH47fhdH8P7vWwihq82lpbpvBXEvdHVDNhC0QZ%2B8iqO%2Boiq7OcaBDspkvR1TiQAdXkbAShu%2FiD6QXltasG%2B32iyMSwMfev121OCG%2BFBlNdfq3JAET%2BEOgJA1Fe2BoY1N94fDQdfyZPpjP%2BhWzxB3mR%2FBwfa92pHrtjjc5Efdeco8Rt1q5YdLuB5u56v5rj%2ByHPJHY4vr%2BONRFfkPpd%2B4QVCtHrt3e7J%2FPBLwxypzwrQX%2FGNSQJNWSY3NLgsA7aDscFjlHI6eqOqSuWuD4aF2rUEB7Sn2auSSb2G3imTKci3h2Pjlu%2FVrkM3vbr8%2B%2Fn7%2FNvj9r5vJf2%2BegMNz%2Feh3va63A0kfQLFrY8eDoc1QA9%2FhzXTVerdB0fh9%2FCeE%2F3s%2FiH%2F5z5%2FgXfgBvs8cFn9ZqW%2BSFGMHBZgRKos5vOKvn7e6%2FrebiE774d5xcB0S%2F696VN1W9%2Fomm3OjOfviXWh8pkyf7YJs1PLir%2BbqwodqpJgb%2BcZxFuwzel%2Fy%2Bt1TECmOAVT9ubl7NGYOae7HpmSapGaAeYXTFE1iEVRN8LOMuRopQGA20yf%2F5WlGyUA4LKvhbnVkpw7tii7nBOjzO6qHjbIb8RwTlC2WHX1kyALRDxFZS84xiaEb4O3u%2BGCpCGqz32sgnORGHxBxzqQYfUn1cz6KPIM6RkAsdxaDOd%2BAjB0JKo8D4Wcy5rFwP%2BvTFu0m6KVtNn2prk5EPxb2VilWo%2BVnI%2F3AiCE0ROF31fNyNm7rNi%2FETs3iy%2Fq%2FbF%2B0RV%2FN8Ko1b4OSNoUKNRp3%2BxVB1Q8KP1XJXT0MuqMDyat6J9QG%2F%2BbWvlnu9lgX0wTLRUaShiQBNQi8b6XcwHNJ3xt%2BphZ9O58%2B1xJDAwduM8d%2Byb8WFBd%2B40RhXnmDMyocytc%2BSRwNdtIVK9b4%2Fb3n8UZpBKtA560%2FaEtJHKle5IWS6KqWdPl%2B2%2FD13VwH68nX94sP4Mvi4ZdfP%2F%2Fvq%2F%2B7Qyc3XE4ZgTxxyogoWm3VtmvuTo5nukeaMUENMxcalVmw6THpt6bg2xEh3xXiG2gbtW0V3wm8ehV%2Fr0TowPeCrjfqD3pOliKvfMFrQKbFsWyf5Jnx%2F0Yi9MsUzHvrOPLrX0sjVlPT%2FjF4NBj2K6a5A5OCsH9EPKqKXp4b%2BYZqxgyEn%2FKZ1pjeARJxkN7C7DlBMHpA3X8O9HreqBH0ekEr0KM%2FCWZEo%2B%2B9Zd0J33FLo3f3%2Fw%3D%3D}{online resource}

==> urls/tree-url.tex <==
\href{https://axa-rev-research.github.io/drawio/src/main/webapp/?chrome=0&grid=0&toolbar=0&p=props&title=Fairness%20Compass#R7T1Zd9s2ur9GZzoP0SEpkZIeHTtOe6dL2mSmTV9yIAqSUFMEA5KW3V9%2FsRMEIYmSqS11Z86JxQUE8O0reoPb1dN7ArLlT3gGk17gzZ56g7teEAwH45D%2Bw648iyvBSF1ZEDQT1%2Fzqwkf0N5QXPXm1RDOY1x4sME4KlMmL8rkYpymMi9qDgBC8rr87x0n9qxlYwMaFjzFImld%2FR7NiKa9Gnlfd%2BB6ixVJ%2Bmk5I3lkB9bS8kC%2FBDK%2BNS4N3vcEtwbgQf62ebmHCtk9tjHjvfsNdPTMC06LNC7%2F8dzrw%2F%2FPTbIjmk%2BAxvLn57x%2F%2FexNIcOTFs1oynNEdkD8xKZZ4gVOQvKuuviW4TGeQDevRX9UzP2Kc0Ys%2BvfgXLIpnCU5QFpheWharRN6d47SQN332u7kUuboclySW83oXzX55T5Z%2Fz2%2F%2BDzx9Wb%2F7HP%2F33ZtI4gQgC1hsWedEPMfWZnxAbtR7iFewIM%2F0AQITUKDHOvSBRKKFfk6%2F%2BgEjOuXAkxj%2FJogmk77nTfR%2FYzGExP83%2Fjjy6oOKJcpxKvDRP4yJVZc4UPcBsNyhR5CUclWfKUG5gP4jmFLyrQEKJGiR0r9jChhI6IVHSApEyeNG3lih2UzgBMzR32DKx2NYkbEF8SWGb3vhXSugb8VQ9mX4VIOLJHr51RpZ1YCqgOP1h17k1wAif70U7PVBh%2FX38Xyew6MA1%2FedgDwy9VJ4kec%2F2Pv9UP38LIfjP%2B6ear%2Be1a8nVPxh%2FP25GoL%2Bql5iP9Q73XGKoCWnGB2FU9wQAp6NByR5bGEko%2BHIZh2%2BZyGRGHUTTkaTgTVCNDwa8%2Fk1uxmtPe8HOP19%2BfNs8uHml9HbN2oJV8t8FIF1wnxGYy%2BsA2TYCfcZ1EftgPvg6V9MmQq8REDljr8e7GRHQ2OSEj%2BuizX5l8KanM8NT6XEBJGttkRDa5gNnMMx2GD3YGLlB7Ah%2BlPi6j5SU2kUFVf6GV8TUxp2xZS8vjcZDLpRgUaTk2k9XgN%2BvSBK6Ja9ndZgGH0tmXHF9%2FlNzjf6hj7g%2B9kT3211n%2F61YP%2B%2B%2B1oCzrNgQjcR4VRAAxXPanw636l6uoExFfdiwFwvUQE%2FZoBT%2Fpqax5YJhJLkFieY8HcH85D9j17PC4IfoHEn4v%2FJVRjXxX%2F78KEGvmwWVsFk7FlE6wcSUdaGHaz0iaVhAg%2B8zbhTQ4Xt8kaR5HZUGJ1d4hyg1B4qpWxIa48Cu%2FlXucrUWlOcssXlD7CIl%2FL%2B4eJJ%2BV12iaegpXiqNKKB70fdcB%2FKy2wpM7KHaS%2BymoNFo3Yia389fzAeWt%2BaeL5FK9v0fGteh7Ddg6RocB7b8wBFrStyO5yCBk0KOqHt6TIuR8F2L9XoxF6qoCHSPxCcUQRBDD2uSDnbKGwPsRhtg%2FEo3qrxpK90wOPrbkqJuC6z8Dweq7ZcQ%2BnDx2cb45Etq4YtGcX%2BcnHi2xqo%2BpZTLnaGoMq4qjiRMgvScjWF5JrcV4raurAU%2FfCF3ioFx%2FGwH0UT479T8Z5hMxTygcAY5dzSe%2BVK7bjSpMmVnM%2B11WWM4MxocJCA25%2B3jH3LMz6Z7OVap3OyB2jJB10GQGCNNbYt6A22RjXWGXy9w4uxvK%2FLFGhLPuO9yWcUdqMdBv5OhGyP3N7wrMi9y7J1Rq3Cppz4DVK5fU1miI68dWGG%2BINxVINiR3bIIHCN2qki4A5LXpURchDvcSLFYNSS%2BYQtmU9rBNjg920JrqZK%2FrGMYwgZOC6SJLdiXSckGQ1UvKXjWHKgnQHWwCcgy%2BvJRXsZeUWXRV5NcXcPUHJdtNVlktg4nFi01ZG8G4b9qJ7UcwyRtxU3DSALSNKPpykuQOEyguvEtSuieYw4pN9wTYcjqTWYccjAEYe0Ey27IxivsVFn4FOHqhOH8ze17tPzt03WRRja%2FsjBYFwf5uDUkpa4EHwDzFPlU3SimER%2BnXkG3fBOf2LzThVvPr5iEk5eCX4rwR8nu%2F6AWLoiR80PvNAqitj%2FnRfHGZw4FTWTmK7RqFGk0VGCbPRCH5aE4eB0MYUmGJVeFWNCVBrZxelVQ8%2FG%2BmHoyO%2FqSK860MccmhhzNdldJ%2BXb23zHO9m2H5xKUfMbToWWZVCu2MvEUvrCoJ1L%2BQB5ElgxaFW9daBoOCjRKlTkXbGY2wTkuSani5QWWwi6I2nhBZZXWimEL8RWlemnOWPg9dWXji9QwsAJz9dY2kv43OBUfC7wRv3J0PdH0XDkheNxZ4E0f2KniapqsCNYum7EVO5rQ2GlKg68JvajjPVOSkl92wPfVXaezX9OxXqiqwqLnbdkS6lOO5PzopPpWFox1zpWS27TGf6MGxziHiQ5ZFuMc8QXdz3MIuowdy6YjG1zqxNeUecUI4r%2Bo5cziwONtehqiz8bBtsBRt8pOMnJ0nwbJSmDzsoBDrKAIleEUjCWFC7EWhkNyhpAUsO8fYsAewH9v3fNjKuz8lBWoVXnWx2pOKNx37Ldxifz2EVnyTLQPEXzkc%2FGnUt1JLXnTf7JeJOdnBjY3p99Mm8tjWlwPJtqHC4G5Onh%2Bf3kpySG93%2FfQQhdZU9NxnZ6xtOW0XSZdOGPQ2dqxEurDU5mPams0evQec5bQ%2BC3LW1S8f2zRxY9WyUaDferGPCGViLLqCXf6gw%2FVaTOqH7Ryo0XC4%2Fy1Sg5Oke7A%2BtsGA47LbOsqmip4XcE9lP8%2FAdZfEreRr99yadr%2F%2Fd89BSqEPyr27hL7tN5HvRh3IfKRpt5nIr7tJlMdDytyYnqjv4vP1dm4AVzsm2E200zH%2B84Lum6yh2MO%2FEztRNbo9GrWtWasR3HQ3RA70I7NLIvv4oiS92KBpO%2Bivvvb%2Bg15hOOTxs8GzWVL6cH68pdT6POqs5YbyBVMHMo9zoBcxq%2Fal37MqfdTXCOo3W5uIyVqvwm8l7CZYZNpnWsxKTQFvRbGWxX6D5uKl7XzKxUuLITP3kdHEEneldQN0tH477qB9Qpa3O6Js%2FS3esF3KXJXLb11Dl96Z3b%2F9ugpzO1R25u%2FDak6KbKTrenfnFZXQc%2BXlfQ%2BwNOUEwfvxfDz2AeE5TxhG5%2BXwUcl4GKHco3qmah1S11MVMX7jADtVcsGfuE6SMiOF1BvrD1EhJ29RmXDIMoeNMZexTzWWQJftYvgiyjn5TVex5aUT7ML6cFejNDbMIrlKrbGZseYsdp0CV5n5bi2RWXPXkBV%2FSfOcErvgvrXnDLYbMoE%2FU%2BJnI6hPdko78XIEU5UE3axGkdCUph3jc2Idu4B%2Fd8RPgEVhnFG%2F5BsSz1JKB%2FLwmc8w1XkdplUbDTP24YeIP7Oemv0QPK4AyBPp0RvcR%2B039%2BxOiLwq0vvSC8pfgW3nhfEkAvZ0RfmeR02%2FkiqqcmX0uUoKnxEPxCEeDLHK5W9B9Y8F9LzH%2BB8ksOUcovUUKgfyf5FwqxMBiBGd1%2FlBdEjM%2Ff%2B5KX5JE%2Bk4CU8jQjAG2yL3X1y5Q%2B9uAIU78LelQeT25vKW%2BlU7yZvPkT0dmQFUhTdfNOgVLDAlSwoLCliyQGFk4xIDP2E88ZDskUDhw%2FcCDFS5Au2GMJXQ8rUhH4kNOtg2%2FwOuWXYrzKKE7wQRHDmXsiVimwl%2B0OfVt%2FglMcBPwK02BCdWdNaTXdgERSC1GcdbM82JiMQijgpiXFoV21FzOkSjjoXZirPAJT2wB5Jg6emaMnJvu6qc%2BIbCebP1F54GZ9hjpsxqzP0Bf3EFe70jKc0uAsgfTDVYSgpYpwnOrVLhrDRuNdxWzNgljrnRcbBk5MaObnsO7NjJ1PSza%2FfInLhLGH6YXEs7fhcyfazcQfn6B1Z6RrYrvWfVTPwynI7dwqwYapQJOKREvdyBpRvN9KU%2FokhFP1HkPHSmplulGsFitxIb6lrNJcCSt9R3nd%2BB0KcUMTKxARFm0mNR8qhryPZbxk7zcmEoNU4rUH5QpBTDAvz8lL1o9%2BQXke1Vc4OQgNqqi%2FN0PzOWS4yT70w1wrfimmCA85XZFnlC4amyckLH2YjToDBRAfEW8vwaMWuzMYU8WMvVCNvgYcscSq5wARqrXl%2FNk51VjkdvK3qf6VCAQplnzfuWIJqZxnuq5YE50rm70A1RyTFd9SA0qxmDlVbVM9BZDn5QrKbY1BmfPtEyRCFYUlyvgWFWvIXxID8e2k%2F64g78YpHgJCQXYgirgjlyy5UIIeYLVxW9deAP6oXDilRcwBHFMxZiyYTrjgC14bfI7p5hQ1CZIYW229BE2KxTSV9kyoIiT0dD5WrsFHqRJBAc0lqICmEIs9z7bcRKXkWTNf%2BoUlH5BOkiB6DeoRBM5Q9pYYBx4QHIvd4IDF8mX5KAcO1%2FTEbHMB7mpENQELWdlefYbcK5uqIfV6hWoozRFFRQrHQS6GQpKE6EYIZMDlYmmvJC8XCyj0S%2FaRNcqlWcHBJ5FPzdREYn6fa6czOn1tbWGCFsx%2B4lgtTCOKCQW9HPNJ1k0sTb%2FbiUpLQ5TGSTnTYF4JXOPYLfY0F1wnxzHin0PpX2UumQKqlpJxBfpWUZRgFdDJb6mmmHCc4V%2FMyrzaQqaYEYqujyiBC74FHME2WXK9gGXLOdj1D6mk6BU1ycQ25VSKA4KwaeJZ8xIL5mq%2FplrxN59pXjK8qqBAjT3KGASCEANtbjmYEbMmPdbFRxsUUyLNjJjZIxyz47gkmosqg8O7kZATH1mkmG14z7a0NQxB%2FJDidcK1RReD5DihdoQTGn%2BQ2YV5Lseq7c4SryEXSLdbyEnN2hyGmdF8P5T4MV%2BGxTLly9BMI66xKsUaNOaXqUIgnDHxWjL0FXRsoDgVLAkQ9CK0CBHIwruJAGkklHXy29H9VnAIKs%2B3IbchVAU3QEJnk7wYxMsN2LzTngy6sSdPYzwOB7YVoE%2BdPIfx6GwcoRLLry8N%2B3ALdNi0QLc267qQBnGqdt9siU6FMNOkk%2Bdz2HMH9ipRKNdJdHqkGk11kCXYxfELu6u2nDbvZCtfu%2BBMm06p8IRNjZwdiOyTDjz7nM6uAsf%2ByC4S3e1Ucrzj73RENbsq%2BS9zRB3koXRkCl52gK3LbkrjRnpDNz4oox3GMYss3AC9srB0W15zto6w7l1WgvLcB2S2pJpOT%2BmdDLyOzqSLOkj%2Bd4n19xyhGVqRsuBeyUeAErHE9v5YexS3J3ajlf8TNaZQyp1fEJBUmGUgWWCCiuWqsssLApAIDU6fpZGaJbBynXGPRVYzCk0fF1%2B2DkmKa3xI8UHp9hGf0oakdDI8C%2FhTC7IwnV55mbEouXJwVHvAJnUHM5jOxODYcBZJ9xLUoyPL3lyUgACK8Wxc9sS8Htqu%2B570qigJlAlbrXRrmEb0CoK8JJDlBGhvnIDrVPh%2FZijPSmXgzkFccOv8e9N%2FIL9qfC%2BjnxQugZoja1mu%2BFpm8jycvLaLK6Vl0BEF%2F6D7WgDuglBvThHg37%2FJm8vMIXmEagQCuVeiCgpDCqEVMCC0wjOY%2FEv4MuKSgLhyZoIkx%2Bo9lniQz%2FnMejVHAyMn7uzQm86hhVMdOaDTn3FPRAPSsqVW5aeSxIUSfgysDDAI7oDk3i9sgmSevFw%2Bl1Ouh%2BZ0m%2FmmK59MDFv41Q53sfEQA18pRfUciWmqCHyclDlFMe4iZu4bxPcQqYUV5Uo4xvn7U5gyti3xb8W5u1gKp%2BcCPEjS5yiAs5zDg%2B%2BGdEtX9%2Bk2YgIo0ilOYPhNvxcYUe17Y1P5dDSrq%2FxqIvEFcLcapX%2B80D6mustuvUTcvaQ8oLxQRKwdpHSAROI8R%2BiKuqVXtsl0OCYsMGZzZO4ogR8VL5Y7RAeThrLArUQM0nSXM1eQ9LD9LvCW0ioFbyFeYCdVzdAjyle7dynFHP4rhh6UsBJ7YjkS5AfqCJLCNVu2cGhz1x%2BdnXhSBTZkPCRLgO2EnpdFSaqIi2AZYiLSZT8VcaBysSwOdcNt7zFyYW44f9w4knZwaW648LzlNfqHkcN%2Bkmz0sKmYb%2B3veiGuuLDZYulMBu2h%2FYK7PJeo6hfcbZLFYNA4BOVIKaZ1luc0bgZbWd436aFzEOcltx33x3ZH2qtxkKlWQVdi6Hd5gtIkGNW9WEE3zKMO1i46kbsYh2oyzqyufaz%2B2nv72vxSLeV5Kw3FEz5RezLX%2Bl%2FNeEpq1qCw1lnolj2ILbNT6%2BlrkQSPUqohk8qDoNTzhnl65SZpbT%2BkbVIZLzLCXbftYlLKSLnIH6F2z0JNWhp%2FBctnEwai4LoqHUJszcEWqCNznxuQOZ4XawHgKsLPPUTqh%2BHCyJa4wBzkiKPQGvP0cwlZDUn2xAKmkJgAadpj0h5dLMTVXHleuG2YC4%2BTmBPIHzjcEryuUk94fgZlLAKFZnBBoN6tmEBVozunl2d45XbyGOZQDquUKj6GoGLtyaFPocqjkykz%2BB23AqW9iOYVKAFzCwkTExk5XxVd4DRReJevRO6%2BSpXj388gtoosmlsoCKlKS7II6SCTLbwik82fDG1JPhw5jkU4b%2BbEeYqOz15AHLU02S4seaJZ%2BX8eFevQpIkuq2SjUfDCrInO89yfskRzwUdAuEt3v7x29witMts%2Fm6nbDTXGGEwrRSrSYSSqJnCBtLYiqEgHTOxERCGiec71A%2BJ6Gn8MiWQ%2FIV6cCddWtCNf4nWVm1krHSxkHq8xeyNiklPWU5ucWZ9ofKC2Qii2WKXy8XlTNQxmBZztnZ76Iyz%2BJZLzM1ksmYMECI7ACtyM0BVWs1Hq4EzL%2FL8wS%2B2XDubUEXnZJGLZzvV0kEvof0pOU%2F3ngSskcM0zVJdYJKgKZzYdGsgkU1BBh%2Bc5a2e4jkupvGdgQKJX1XEwgIntYN%2BkE%2Fwiv6X3snqiV%2BWK1pRm6EL8Q7WE6Iq0hCDyhn3P7tI%2FUGXIF6MoqILB61AUztvPv%2B3Rvd23WHqZP7jpwLmCs4G2YmsnikY4HBzDM%2Bx7pzjA1709wTUS83n6oDmI2d3A%2BGQpnhPV60I3IOuso35L9GnmcF%2Fw6T1bKaAbSyS0Ott34%2F0dWBHfQXi0Ct1fyiLj%2FsfiOYP7GCz1F1vZKawmKhfoItMwxKYXKC1xmWu8EjWu80KG%2B5Ud4Wmt3dcVWtyaEQq%2FmZSkS3qnVcqNWV%2BYWS2LueZbuXexWhuoJCC1bqiFAmamXq7zrsRq2CzKFKymaCHXoxzS%2BvNCUzey0PjnNzc6OcCJKku62MwxkPkrBD860nuADQ%2B15xn3ZEtvOWQltZXHVILIXIMaI4Hg0egDYrRakQ5Aw7GZMNlhNi2R9iTB3PybV01i6GSKKr%2FHkZbmhAWVQdTUYqyF%2BzNlOeqmtDqkU4Bwmoh8xBUgD1AmzbgKD%2BO6giTN7mm1UeYmYpNYDjVuRtdk3IwjS1RNlM57AsPmldFdHaN7ZWn%2FRJY2viaW1kjEOzdLU5ueZxzO7Q6rarQAe8fQX%2FlOmx1adMh5hXnhO2U8mqVw16YOTzOear9t4IWYpYkabVrhkYqxcAT%2FDcY8KtmGDX%2BkM38w82QJBwkLksumaQbTzYwvCeZL5KcqFs6y1t%2BwQn3Z4YIaCitFaqtGJQMjbnP%2BKmRdsZM5AbXgruLWkr552i4nNsaS2YwdiQ2iF414Q77eN%2FbJbJ5if67R4Gb7l2RhhIgpz1hGwBzx2QHhCOdl8d73%2FGHOy7jPW2AXNIYTmQNYpLhz7MrVPFeC627GsRrDXSCRESx4OfNWG1nPkqWxPnpfS5ga0QxQX7FKj%2Bb7InuqsEeqjtpsMRnvXCC2aEUZkXC76%2B%2BwMopHNNPNI2QXoFW2FC1HVG4CZemZbIJjr8uUVriGkY1V1QWD7swyhSmcI931QD%2FOtlN6%2FAtO441JV9EKJlfRjIOVZbj3dHaMSt02OqIwmbOQEmTTSjZBVBBXJ9ULFK3LGaevQudKVOJNt8GkmF2qLoJU0iGzukiHaFD6yKI0CxmlET2WzBYXtYiSbPAhslPQClUaWVqytkIK49YEpwtON3nJ4S%2BaHFKErWU6UekqdmsFnuhoOexZbIlnwX9V5L5EvHNNQrWHpKfzT4QQLaci3lbVN%2FR2K0%2BSS%2BC4FNlMC0BkDZMB3dpuiKQiyWpuKxRTXXbEp2TpRrpt9nyf2ASrhh6MLos1czc%2B98wgGfuhmpMYGSoHp5ZsL16%2FMCVkMKk7nIwq7zNpIe8IEQYH1QNzh%2F7QUBvsJ5paRNuYuevLbZrA1Vra1Aep9euqN%2Bqq2IVsSWP3LK%2FlLM6bBzOwzDNGkBuqAysxJg1Drk2Y8%2BvVdPIWwtIZ4z2kD1MLO0IzWsZqRGAby25LyIiUz2r8tpYBYDZtUi2cOF8gkLIJUS5G%2Bckc6XSAqg5OqwYOsKi%2BPt%2Bxr5n6INCTUWltdBFYw1mWHSVowSqb%2Fm3yHSunwYCKyChQSQbcnMKC%2FzUVMa2SVJ9XaoJjwWaLKoZGv1igZeTON%2B%2B2Z1jMc1Fita2kTepiNiXU2m0anDvhqQc1cUOZtF5L%2FiBUDzbKFpZcYJwUKFO0vZNL%2B941semRb2UAjibfhK3YPa%2Fv2mJ8FQqvQuFVKFypUNguAYJrkgD6sHslAYaj00mARjR%2F6wmWRjRfgYbt0eFi4ncVr5AOZeSUFTajaisr2GkNfHom5nSBCJ3A3bO7Jh5V8u%2BuBnUmQVxsvzZ9r8s6AOcWSF%2F%2B7lS9XsfJPYfrcB8%2F3fz2qbUi9JEurWinAL1VjifRWDqWKiKRtUqcqRsKhOwrDiuxzXuycuXIaGfdzBK%2Br8a4ZSd85BtThVV3DfGpnOJSUilZhiCExVJ2LvlaMsedEJ9mQ3PlJGbhV%2FhUaF0igWBWfUEoeLJGjyux9bbbm%2FrPir2RnzIEaLsw5y19nNWQGfoeXZpq1WN4cFkLYQKqKOK8JFK48%2FRpkfpe%2BRKp0jgvk54OB7YRuZuJZLPErXGBczDbxvkmgadaA%2BzitnZvxGOlTzu6oDUklsjcf8ke7Z%2B8Fvh2hkbgUFCCgWProv23rt3JgJFrr6Ra0Fob4XRmKSQfZIznUSutPFVC08TUJtGXfc7UZToYpj5BW9vRROi3IEKUJLc4oTyEvTuYh%2Bx%2FzCtQEPwAjTsR%2F0%2FO1bgu%2FmuFqtupoTWRBw7taeJASvuQzEOQ0nmy9qiBkx%2B%2B692GvbcR31Q6vxGzrUQ%2BMzezbtifzDLkj3ttHvf%2F3QAsl1Y7IdrIqD0%2BYJ7rG76LW3QBGPeUwwZkLoOzRoFlAuhzos%2FGWUeuveqcs9L9fOWr5%2BGrm06daqLpKejVyUib3oYP332uMUWTTzoZ6e7Hz89I20PiUhipErEXx0jHaiJVd6PA0UchPCUnHW%2FWUekHeKLvEpDcOn%2BzLObMmDKTQ1%2FMvjaGcmLBV9ggZDH9LpTkUf37bzEF%2FsE5WKHkWTxNre5HyDJMjfuOCckb4rvsTorJCiTGvbWEBLs59EQIgVrc7HirN3TaMfO3N95kdPoGpTOOSeymp77H7xQEpDk%2FoEq%2BmUJxl%2FV7qY%2BqX5yC%2BEG0GHpjbUowHIvdCIYT%2BUfoyX1hHXETIPcEiQCHWFuCQWF9viEQv9sYwXoF2zHB1iATIR1egXF9NET%2FBSsmbdJpzv4R4r5pVr3C9pXQ%2FuHAOBahMT16SyLG2dRrrau%2BRL12aowHqNfbEm1eZunewRVe0E1c8tKLbXZ1y2jQjgF3ZscsMNBpujPnWI5jF%2BbgEZdEpj3gsohFQVQ9h4C1KFykVSwJAnF8n0xhVh8VByek9XK2npkU3TMOCWVV4nIh7MUlgfMaHJZFkeUcBvf0%2F4A8occ%2BJgv295SOeu%2F73rA%2FmLAIuaGz62Dhl2kC0gcH2FgfHApWkxsCvbPh3e4wzOZeZC3CMNfgqdiDgI9AsQeFcLRJe2n2cRRNmh2EXCby0ZyN7v3qNOS1HSSH7%2BLZfLHNVn7dyIxbdRqJKO1gFaZ5IaPjuz2zGxU0rs9I8X3DNaN5sV3lOr7bdqtCcmX8cO%2BImPIwmgjsinB34S90u8Ca7aIUbGbocTMSOdXlw7TefXFG5rPFGm7VgwqCpqCfg7g%2B%2F8rY6MaH54wJUgjcwfYhROvxmsZeT5Drmvw4lC%2FDHLi%2BsGXgop4L0Cb8iZ1M4wxbujjN0URleKyw5VtdAS4SqoyEfGlYvMYwTy4JhxtwebMkdJj24yPRsjOk2TxH5x21PD%2F2NiWFcBNQ8vStT%2Fr8yfOy1vbg2MJaj6WYuKd8qRkh%2FqgFa3WmNR2PtW5W4rplrXYLolfWegbW2j4pQd6dNNFzdErO6rt8Lq82xj543BQwfmtR5Nui6J9nWXSRx9NVpurxAg3veDL036Kl12x2zdy5TXHw5tVujYDw0MamGhDVSsYMRBSkdJcBi%2BtW%2FW83IYvI9%2FqUj22KWVRXN0UvvgdkVnQfvYh2VO5fqiQ9qB7Fyvx11VT46sS4I8cynHK1qSFvTE9%2F3i%2Bb%2FbnuivJ674LeeNxjiq73bPwe87feMmPH741OaOUc1MbBiq4EjmY7wXUx%2BSzDpODdzOA%2FidtvWPZutq%2B7%2F7EKzyc%2BGEWh3Oijp96sKhjNL%2F9SlzO1MkfVHUGeuiZLAGXJvepQYPZz3RBRF00ACJU%2BiFjNFHRngG9XvphU%2FG3Ll6HyeG2VLx25wA6SL1F7%2BbIpyX%2F346dM8j8EStapIW6p0VHQ4XhS45bu1pTIfiDn5%2BaO6bRJXBL7I3RtbJyEuUmb5zeVGt%2FQ3w3FPTMrnzi%2BV8xadkAx0pWqdowfS9nL21hO1UNGd27syYareYbTme5BpCemO36jqrGpbNBK%2F%2FpO9pqWVxh1Nc6CFQuKVS8g3XxSNqxZIvhYHQvKCUf1ghS9dNi5a5iSxbMeS93BK5TnxoGz%2B0ufrJyu4KyfxlPUT5NVP0XL%2FgI%2F0jvBYOKNRmOfP3eYGLoleJ3j9AiCaEcnyW9HEA08u8TRKYiiMwqiV%2F9h78U5CvVyu4%2F0V96qMM96smEO5j3LHAylOfitexoPobSxTWkuZcKl8h3Q4cKlTHwSPeZkzzV59IQQInv0at0ySithLvtfy04raAa5GEyx2c%2Fc7kGtG2ODKeZHFdgfVq3wqCgrCJqW4uptz9Xihp%2BoPa%2BsNLpmZWtt2aAbQ2aLntCSLkR35UTM1jx4guKPfUmrBJygRVCNYGbPqmQ%2F1dLiJf201YmmVE0oV6plH9UeSImKlWiLWG8XbZ04IY%2Bv4DqE6P2t2vVJ1%2BfaaOfHOuUY56DK7oCiW%2FUjkm0ExRubR5HvimM4KAk%2BIrjuVZ3Kc5YAySG2gJSrkzqGTIFoO4h1W%2BoKRGwe99v2WbbTK4yvTYVflx3JIY6B5ViD2Gq44S7UwPpisOycuKldkKlxOJtTDbYrHJfVEW%2BszkDXqcqhq7nHqVriObWGwGG%2BSuemXXS%2ByT26%2B%2FFvxj06aTS6CI%2FnHm15QuGxMsbq2dWiLSuI45KAmOVV18qo7A5D%2F%2BiEhEM4xaRZ19C6h0oXqDUOFwPy9PD8fvJTEsP7v%2B8ghF20yxxErnaZBoK26JPXcNQ3VGU3xzjSMZyst2MuEaDHywhYaeMn0QfS60oL9u2umpVxaeDDYNiNGtwSH5qs5kadP5LiGdwDELKmojswdLHp%2FmgU9i1Ppj%2Fxg37zhHKX%2BREcbd%2BbHbnuqkNSvtWdp8xj3G9WfriE6%2FF2vpnv%2Bi3LIX88sbiOPxk3kf9Y%2Bo0bBM3qsXu3J%2FvbIwF%2FojInTHvBPyUFtGmV1NrssgDQDcqORk3O4eiJqi6ZuxaOjrVrLQpoz7FXY5d8i%2FpNJFOWaw3HJi%2FfrR%2BCYvHu7vfHX%2B%2FfB79%2BvZ3%2B7%2FYJODzXj37f63t7kPQRFLsudjwY2Qw18B3eTFetdxcU%2Fecvf47AOP71U3EzK%2Fz8zy93X%2F907LahTBQE8pCY4SuyGmbshkldlslWHKbgk5fasmMXodQ7MZuycNgZ6OwTbVT74FqVvmY%2BJ4Fd01vzogyXwPeCvjcehgOnjSavfMJrQGbVuR2%2FyUNF%2F4OET485bu%2Bt8ypvfqiN2Iw5%2FmPQKIyGNs91IFIQDU%2BIRk27nse832LCwwi%2Flbz%2FCIfuT4DEHKJ3sHhOEYwfUP%2BfA7xgMm4DvEHQCfDoT4JxYdx7z5rO%2FEQNPPbE%2FwM%3D}{online tool}
